Persistent homology of partially ordered spaces

In this work, we explore links between natural homology and persistent homology for the classification of directed spaces. The former is an algebraic invariant of directed spaces, a semantic model of concurrent programs. The latter was developed in the context of topological data analysis, in which topological properties of point-cloud data sets are extracted while eliminating noise. In both approaches, the evolution homological properties are tracked through a sequence of inclusions of usual topological spaces. Exploiting this similarity, we show that natural homology may be considered a persistence object, and may be calculated as a colimit of uni-dimensional persistent homologies along traces. Finally, we suggest further links and avenues of future work in this direction.

==> macrosPersAPCT.tex <==
%%%%%%Macro texte%%%%%%
\newcommand{\pdf}[1]{\texorpdfstring{$#1$}{1}}

\makeatletter
\def\@equationname{equation}
\newenvironment{eqn}[1]{%
    \def\mymathenvironmenttouse{#1}%
    \ifx\mymathenvironmenttouse\@equationname%
        \refstepcounter{subsubsection}%
    \else
        \patchcmd{\@arrayparboxrestore}{equation}{subsubsection}{}{}%          doesn't change output?
        \patchcmd{\print@eqnum}{equation}{subsubsection}{}{}%
        \patchcmd{\incr@eqnum}{equation}{subsubsection}{}{}%
%       \def\print@eqnum{\tagform@\thematrix}%                          instead of etoolbox' \pathcmd
%       \def\incr@eqnum{\refstepcounter{matrix}\let\incr@eqnum\@empty}% instead of etoolbox' \pathcmd
    \fi
    \csname\mymathenvironmenttouse\endcsname%
}{%
    \ifx\mymathenvironmenttouse\@equationname%
        \tag{\thesubsubsection}%
    \fi
    \csname end\mymathenvironmenttouse\endcsname%
}
\makeatother


\newcommand{\I}{\mathbb{I}}
\newcommand{\Ifl}{\leftarrow}

%%%%%%%%
%% XYPIC %%
%%%%%%%%

%% Options 
%\renewcommand{\objectstyle}{\displaystyle}
%\renewcommand{\labelstyle}{\displaystyle}
%\UseTips
%\SelectTips{eu}{11}

%% Nouvelle direction pour les monomorphismes (>->)
%\newdir{ >}{{}*!/-10pt/@{>}}
\newdir{ -}{{}*!/-10pt/@{}}
\newdir{> }{{}*!/+10pt/@{>}}

%%%%%% 4-cellules%%%%%%%
\makeatletter

% Noms des nouvelles directions
\xyletcsnamecsname@{dir4{}}{dir{}}
\xydefcsname@{dir4{-}}{\line@ \quadruple@\xydashh@}
\xydefcsname@{dir4{.}}{\point@ \quadruple@\xydashh@}
\xydefcsname@{dir4{~}}{\squiggle@ \quadruple@\xybsqlh@}
\xydefcsname@{dir4{>}}{\Tttip@}
\xydefcsname@{dir4{<}}{\reverseDirection@\Tttip@}

% Commande quadruple
% Attention : la position des pourcents est importante !!
\xydef@\quadruple@#1{%
	\edef\Drop@@{%
		\dimen@=#1\relax
		\dimen@=.5\dimen@
		\A@=-\sinDirection\dimen@
		\B@=\cosDirection\dimen@
		\setboxz@h{%
			\setbox2=\hbox{\kern3\A@\raise3\B@\copy\z@}%
			\dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
			\setbox2=\hbox{\kern\A@\raise\B@\copy\z@}%
			\dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
			\setbox2=\hbox{\kern-\A@\raise-\B@\copy\z@}%
			\dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
			\setbox2=\hbox{\kern-3\A@\raise-3\B@ \noexpand\boxz@}%
			\dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
		}%
		\ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \noexpand\styledboxz@
	}%
}

% T�tes de quadruples fl�ches : positionnement ok, reste la jointure
% Les parties comment�es sont des essais � reprendre plus tard
\xydef@\Tttip@{\kern2pt \vrule height2pt depth2pt width\z@
	\Tttip@@ \kern2pt \egroup
	\U@c=0pt \D@c=0pt \L@c=0pt \R@c=0pt \Edge@c={\circleEdge}%
	\def\Leftness@{.5}\def\Upness@{.5}%
	\def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
	
\xydef@\Tttip@@{%
	\dimen@=.25\dimen@
%	\A@=-\sinDirection\dimen@
 	\B@=\cosDirection\dimen@
	\setboxz@h\bgroup\reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@
%	\kern\A@ \raise\B@ \boxz@ \kern\L@c
%	\kern-\L@c \boxz@ \kern\L@c
	{\vDirection@(1,-1)\xydashl@ \xyatipfont\char\DirectionChar}%
	{\vDirection@(1,+1)\xydashl@ \xybtipfont\char\DirectionChar}%
}

% Red�finition de la commande \ar 
% Provoque un avertissement � la compilation
%\xydef@\ar@form{
%	\ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@form}%
%	\else\ifx ^\next \DN@ ^{\xyFN@\ar@style}\edef\arvariant@@{\string^}%
%	\else\ifx _\next \DN@ _{\xyFN@\ar@style}\edef\arvariant@@{\string_}%
%	\else\ifx 0\next \DN@ 0{\xyFN@\ar@style}\def\arvariant@@{0}%
%	\else\ifx 1\next \DN@ 1{\xyFN@\ar@style}\def\arvariant@@{1}%
%	\else\ifx 2\next \DN@ 2{\xyFN@\ar@style}\def\arvariant@@{2}%
%	\else\ifx 3\next \DN@ 3{\xyFN@\ar@style}\def\arvariant@@{3}%
%	\else\ifx 4\next \DN@ 4{\xyFN@\ar@style}\def\arvariant@@{4}%
%	\else\ifx \bgroup\next \let\next@=\ar@style
%	\else\ifx [\next \DN@[##1]{\ar@modifiers{[##1]}}%]
%	\else\ifx *\next \DN@ *{\ar@modifiers}%
%	\else\addLT@\ifx\next \let\next@=\ar@slide
%	\else\ifx /\next \let\next@=\ar@curveslash
%	\else\ifx (\next \let\next@=\ar@curveinout %)
%	\else\addRQ@\ifx\next \addRQ@\DN@{\ar@curve@}%
%	\else\addLQ@\ifx\next \addLQ@\DN@{\xyFN@\ar@curve}%
%	\else\addDASH@\ifx\next \addDASH@\DN@{\defarstem@-\xyFN@\ar@}%
%	\else\addEQ@\ifx\next \addEQ@\DN@{\def\arvariant@@{2}\defarstem@-\xyFN@\ar@}%
%	\else\addDOT@\ifx\next \addDOT@\DN@{\defarstem@.\xyFN@\ar@}%
%	\else\ifx :\next \DN@:{\def\arvariant@@{2}\defarstem@.\xyFN@\ar@}%
%	\else\ifx ~\next \DN@~{\defarstem@~\xyFN@\ar@}%
%	\else\ifx !\next \DN@!{\dasharstem@\xyFN@\ar@}%
%	\else\ifx ?\next \DN@?{\ar@upsidedown\xyFN@\ar@}%
%	\else \let\next@=\ar@error
%	\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}

\makeatother

\newcommand{\bigslant}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{ $\scriptstyle #2$}\right.}}



%%%%%%Macros locales%%%%%%%%%
\tikzset{%
    triple line/.code={\tikzset{%
            double equal sign distance, % replace by double distance = 'measure' 
            double=\pgfkeysvalueof{/tikz/commutative diagrams/background color}}},
    quadruple line/.code={\tikzset{%
            double equal sign distance, % replace by double distance = 'measure'
            double=\pgfkeysvalueof{/tikz/commutative diagrams/background color}}},
    Rrightarrow/.code={\tikzcdset{triple line}\pgfsetarrows{tikzcd implies cap-tikzcd implies}},
    RRightarrow/.code={\tikzcdset{quadruple line}\pgfsetarrows{tikzcd implies cap-tikzcd implies}}
}    

\def\eg{{\em \emph{e.g.}}}
\def\cf{\emph{cf.}}
\def\ie{{\emph{i.e.}~}}

%\newcommand{\set}[1]{\{#1\}}

\newcommand{\longannotatedarrow}[1]{\overset{#1}{\longrightarrow}}

\newcommand{\dual}[1]{\overline{#1}}
\newcommand{\norm}[1]{\hat{#1}}
\def\square{\vcenter{\hbox{$\scriptstyle\oblong$}}}
\newcommand{\indicator}[1]{\iota^{#1}}
\newcommand{\Ver}[1]{V({#1})} 
\newcommand{\Edg}[1]{E({#1})} 
\newcommand{\web}[1]{\mathcal{W}(#1)}
\newcommand{\redrel}{\longannotatedarrow{}{R}}
\newcommand{\critminmeas}{\nu}
\newcommand{\critmaxmeas}{\mu}
\newcommand{\redmeas}{e_{\vlan}}
\newcommand{\greenmeas}{e_{\vlor}}
\newcommand{\numand}{\#_{\vlan}}
\newcommand{\myrightleftarrows}[1]{\mathrel{\substack{\xrightarrow{#1} \\[-.9ex] \xleftarrow{#1}}}}
\definecolor{mred}{rgb}{0.7,0.1,0.1}
\definecolor{mblue}{rgb}{0,0,0.8}
\definecolor{mgreen}{rgb}{0,0.6,0.3}

\newcommand\natlax[0]{\Phi}
\newcommand\laxnat[0]{\Psi}
\newcommand\gplax[0]{\Gamma}
\newcommand\laxgp[0]{\Lambda}
\newcommand\Fact[1]{{F}#1}
\newcommand\RFact[1]{{\mathcal{R}}#1}
\newcommand\LFact[1]{{\mathcal{L}}#1}
\newcommand\threemap[3]{#1: #2 \Rrightarrow #3}
\newcommand\Driag[1]{\mathbf{Diag}(#1)}
\newcommand\Pairs[1]{\textbf{Pairs}(#1)}
\newcommand\diagiso[1]{\textbf{Diag}_{iso}(#1)}
\newcommand\diagab[0]{\textbf{Diag}(\textbf{Ab})}

\newcommand\gpo[1]{((#1),\mu,\eta, (-)^{-1})}

\newcommand\fcat[1]{\overrightarrow{\boldsymbol\Pi}(#1)}
\newcommand\trace[3]{{\mathfrak{T}}(#1)(#2,#3)}
\newcommand\trac[2]{{\mathfrak{T}}(#1)(#2)}
\newcommand\disctrace[3]{{\mathfrak{dT}}(#1)(#2,#3)}
\newcommand\dtrace[3]{\overrightarrow{\mathfrak{T}}(#1)(#2,#3)}
\newcommand\syst[1]{\overrightarrow{\mathbb{T}}(#1)}
\newcommand\sysh[2]{\mbox{$\overrightarrow{H}_{#1}(#2)$}}
\newcommand\sysinth[2]{\overrightarrow{h}_{#1}(#2)}
\newcommand\syshhm[2]{\overrightarrow{H}^{HM}_{#1}(#2)}
\newcommand\syshd[2]{\overrightarrow{h}_{#1}(#2)}
\newcommand\syshdhm[2]{\overrightarrow{h}^{HM}_{#1}(#2)}
\newcommand\sysc[2]{\overrightarrow{\mathbb{C}}_{#1}(#2)}
\newcommand\sysp[2]{\overrightarrow{P}_{\!\!#1}(#2)}
\newcommand\syspi[2]{\overrightarrow{\Pi}_{#1}(#2)}
\newcommand\Cr{\mathcal{C}}
\newcommand\Dr{\mathcal{D}}
\newcommand\Er{\mathcal{E}}
\newcommand\Kr{\mathcal{K}}
\newcommand\Br{\mathcal{B}}
\newcommand\Real[0]{\mathbb{R}}
%\newcommand\Real[0]{\mathbf{R}}
\newcommand\M[0]{\mathcal{M}}
\newcommand\mon[0]{\textbf{M}}
\newcommand\N[0]{\mathbb{N}}
\newcommand\E[0]{\mathcal{E}}
\newcommand\lF[0]{\mathcal{F}}
\newcommand\V{\mathbf{V}}
\newcommand\G[0]{\mathcal{G}}
%\newcommand\T[0]{\mathcal{T}} 
\newcommand\HT[0]{\mathcal{HT}} 
\newcommand\fc[1]{F_{\Cr}[\Sigma_{#1}]}
\newcommand\twoB[0]{\Br^{2}}
%\newcommand\A[0]{\mathcal{A}}
\newcommand\Lim[1]{\mathcal{L}_{#1}}
\newcommand\PP[0]{\mathcal{P}}
\newcommand\diP[1]{\overrightarrow{\mathbf{P}}\!(#1)}
\newcommand\discP[1]{\overrightarrow{\mathbf{dP}}\!(#1)}
\newcommand\tpos[1]{{\mathbb{P}}(#1)}
\newcommand\diG[1]{\overrightarrow{Geom}(#1)}
\newcommand\ob[1]{Ob(#1)}
\newcommand\iar[1]{\lfloor#1\rfloor}
\newcommand\quo[1]{#1/(\sim_o,\sim_m)}
\newcommand\vq{\mathcal{V}-\textbf{QCat}}
\newcommand\abq{\textbf{Ab}-\textbf{QCat}}
\newcommand\digeom[1]{\overrightarrow{Geom}(#1)}
\newcommand\quot[2]{{#1}/{#2}}
\def\Z{\mbox{$\mathbb{Z}$}}
\newcommand\diC[2]{\overrightarrow{C}_{#1}(#2)}
\newcommand\diCr[3]{\overrightarrow{C}_{#1}^{#3}(#2)}
\newcommand\Rightarrowstar[0]{\overset{*}\dfl}
\newcommand\Leftarrowstar[0]{\overset{*}\Leftarrow}
\newcommand\kernel[1]{ker(#1)}
\newcommand\cok[1]{cok(#1)}
%\newcommand\im[1]{im(#1)}
\newcommand\coim[1]{coim(#1)}
\newcommand\Kernel[1]{ Ker(#1) }
\newcommand\Crok[1]{Cok(#1)}

\newcommand{\tr}[1]{\overline{#1}}
\newcommand{\fl}{\rightarrow}
\newcommand{\dfl}{\Rightarrow}
\newcommand{\tfl}{\Rrightarrow}
\newcommand{\qfl}{\xymatrix@1@C=10pt{\ar@4 [r] &}}
\newcommand{\Xr}{\mathcal{X}}
\newcommand{\Vr}{\mathcal{V}}
\newcommand{\Yr}{\mathcal{Y}}
\newcommand{\Ar}{\mathcal{A}}
\newcommand{\Tr}{\mathcal{T}}
\newcommand{\dcyl}[1]{#1 \times\!\! \uparrow\!\! I}
\newcommand{\cyl}[1]{#1 \!\times \!I}
\newcommand{\dI}{\uparrow\!\! I}

%% Catégories

\def\catego#1{{\bf{\sf #1}}}
%
\newcommand\cat{\catego{Cat}}
\newcommand\catsigmab[0]{\cat_{\Br_0}/ \Br}
\newcommand\catsigma[0]{\cat_{X}}
\newcommand\catxp[0]{{\cat_{X}/ \diP{\Xr}}}
\newcommand\catx[0]{\cat_{X}}
%
\newcommand\ab{\catego{Ab}}
\newcommand\gp{\catego{Gp}}
\newcommand\gpos[1]{\gp(#1)}
\newcommand\abo[1]{\ab(#1)}
%
\newcommand\act{\catego{Act}}
\newcommand\Vect{\catego{Vect}}
%
\newcommand\setcat{\catego{Set}}
\newcommand\psetcat{\setcat_{*}}
%
\newcommand\natsys[2]{\catego{NatSys}(#1,#2)}
\newcommand\natsysnu[2]{\catego{NatSys}_{\nu}(#1,#2)}
\newcommand\laxsys[2]{\catego{LaxSys}(#1,#2)}
%
\newcommand\opnat[1]{\catego{opNat}(#1)}
\newcommand\opnatnu[1]{\catego{opNat}_{\nu}(#1)}
\newcommand\diag{\catego{Diag}}
%
\newcommand{\Top}{\catego{Top}}
\newcommand{\potop}{\catego{PoTop}}
\newcommand{\dtop}{\catego{dTop}}
%
\renewcommand{\split}{\catego{Split}}

\newcommand{\Ch}{\catego{Ch}}
\newcommand{\pmCh}{\catego{pmCh}}
\newcommand{\mCh}{\catego{mCh}}
\newcommand{\dCh}{\mathcal{F}}
\newcommand{\mdCh}{\catego{m}\mathcal{F}}

\newcommand\tck[1]{{#1}^\top}

\newcommand{\colim}[1]{\underset{#1}{\mathrm{colim}}}


%%%% Glob Posets
\newcommand{\Hasse}{\mathcal{H}}
\newcommand{\Mol}{\mathcal{M}ol}
\newcommand{\SMol}{\mathcal{SM}ol}
\newcommand{\Glob}{\mathcal{G}l}
\newcommand{\glSet}{\mathbf{gl}\mathbf{Set}}
\newcommand{\poCat}{\mathbf{p}\omega\mathbf{Cat}}
\newcommand{\oCat}{\omega\mathbf{Cat}}
\newcommand{\cl}[1]{\textit{cl}(#1)}
\newcommand{\Del}[2]{\Delta_{#1}^{#2}}
\newcommand{\del}[2]{\partial_{#1}^{#2}}
\newcommand{\Pos}{\mathbf{Pos}}
\newcommand{\Posin}{\mathbf{Pos}_{in}}
\newcommand{\ogPos}{\mathbf{ogPos}}
\newcommand{\GlobPos}{\mathbf{GlobPos}}
\newcommand{\Globe}{\mathbf{Globe}}
\newcommand{\Pol}{\mathbf{Pol}}
\newcommand{\RPol}{\mathbf{RPol}}
\newcommand{\rPol}{\mathbf{rPol}}
\newcommand{\RDCpxin}{\mathbf{RDCpx}_{in}}
\newcommand{\RAtomin}{\mathbf{RAtom}_{in}}
\newcommand{\skel}[1]{\sigma_{\leq #1}}

\newcommand{\D}{\overline{D}}
\newcommand{\DD}[1]{\overset{\Rightarrow}{D^{#1}}}
\newcommand{\Gl}{\overset{\rightarrow}{Gl}}

\newcommand{\ei}{\underline{\iota}}
\newcommand{\ef}{\underline{\sigma}}
\newcommand{\de}{\partial}
\newcommand{\vI}{\vec I}
%\newcommand{\p}{\times}


%Kleene Algebras
\newcommand\KA{\catego{KA}}
\newcommand\KAT{\catego{KAT}}
\newcommand\KAD{\catego{KAD}}
\newcommand\KACD{\catego{KACD}}
\newcommand\MKA{\catego{MKA}}
\newcommand\MKAC{\catego{MKA}^\lor}
\newcommand\exh[0]{\catego{exh}}
\newcommand{\dom}[0]{\mathit{d}}
\newcommand{\cod}[0]{\mathit{r}}
\newcommand{\adom}[0]{\mathit{ad}}
\newcommand{\acod}[0]{\mathit{ar}}
\newcommand{\conv}[1]{{#1}^{\lor}}
\newcommand{\op}[1]{{#1}^{\mathit{op}}}
\newcommand{\con}[2]{{#1}^{\lor_{#2}}}
\newcommand{\inv}[2]{{#1}^{{-1}_{#2}}}
\newcommand{\Rel}[1]{Rel(#1)}
\newcommand{\fDia}[1]{| #1 \rangle}
\newcommand{\bDia}[1]{\langle #1 |}
\newcommand{\fbDia}[1]{\langle #1 \rangle}
\newcommand{\fBox}[1]{| #1 ]}
\newcommand{\bBox}[1]{[ #1 |}
\newcommand{\fbBox}[1]{[ #1 ]}
\newcommand{\modalops}[1]{\fbBox{\fbDia{ #1}} }
\newcommand{\ud}[1]{ UD(#1) }
\newcommand{\pt}[1]{ PT(#1) }
\newcommand{\mult}{\odot}
\newcommand{\un}{\mathbbm{1}}
\newcommand{\abs}[1]{ \mid \! #1 \!\mid }
\newcommand{\noeth}[1]{\mathcal{N}(#1)}
\newcommand{\noethi}[2]{\mathcal{N}_{#2}(#1)}

%ARS
\def\lfl{\leftarrow}
\def\rfl{\rightarrow}
\def\refl{\overset{\equiv}{\rightarrow}}
\def\invrefl{\leftarrow^{\!\!\!\!\equiv}}
\def\sym{\leftrightarrow}
\def\symtran{\overset{*}{\leftrightarrow}}
\def\tran{\overset{*}{\rightarrow}}
\def\ltran{\overset{*}{\leftarrow}}
\def\red{\twoheadrightarrow}
\def\invred{\twoheadleftarrow}
\def\rst{\overset{\ast}{\leftrightarrow}}
\newcommand{\rep}[1]{#1}
\newcommand{\rrs}[1]{#1^{c}}

%SRS
\def\drst{\overset{\ast}{\Leftrightarrow}}
\def\drstl{\overset{\ast}{\Longleftrightarrow}}

%Completion
\def\KB{\mathcal{KB}}
\def\nf#1{\text{NF}(#1)}
\def\irr#1{#1^{\text{nf}}}
\def\Sr{\mathcal{S}}


%Persistence 
\newcommand{\PersCat}[2]{{#1}_{pers}(#2)}
\newcommand{\Pers}[1]{\catego{\textit{Pers}}(#1)}
\newcommand{\iPers}[1]{\catego{\textit{IsoPers}}(#1)}

\newcommand{\real}[1]{|| #1 ||}




